Closing the Knowledge Gap in Designing Data Annotation Interfaces for AI-powered Disaster Management Analytic Systems

Data annotation interfaces predominantly leverage ground truth labels to guide annotators toward accurate responses. With the growing adoption of Artificial Intelligence (AI) in domain-specific professional tasks, it has become increasingly important to help beginning annotators identify how their early-stage knowledge can lead to inaccurate answers, which in turn, helps to ensure quality annotations at scale. To investigate this issue, we conducted a formative study involving eight individuals from the field of disaster management, each possessing varying levels of expertise. The goal was to understand the prevalent factors contributing to disagreements among annotators when classifying Twitter messages related to disasters and to analyze their respective responses. Our analysis identified two primary causes of disagreement between expert and beginner annotators: 1) a lack of contextual knowledge or uncertainty about the situation, and 2) the absence of visual or supplementary cues. Based on these findings, we designed a Context interface, which generates aids that help beginners identify potential mistakes and provide the hidden context of the presented tweet. The summative study compares Context design with two widely used designs in data annotation UI, Highlight and Reasoning-based interfaces. We found significant differences between these designs in terms of attitudinal and behavioral data. We conclude with implications for designing future interfaces aiming at closing the knowledge gap among annotators.

==> 99_02_related_work_backup.tex <==
\section{Related Work}
%connect literature in group work and data annotation user interface. 
In this review, we first describe how knowledge gaps between group members can impact group work and what common approaches exist to mitigate such gaps.
We then examine data annotation user interface studies.
By synthesizing insights from both directions of review, we conclude the review with the necessity of more deeply understanding knowledge gap-driven design in data annotation user interface research.

All forms of collaboration stem from a similar motivation; group work can be productive because it allows individuals to share and gain insights they might not have discovered independently~\cite{cabrera2006determinants}. 
By pooling the knowledge and expertise of all members, group work can be executed more efficiently and accurately~\cite{austin2003transactive, hong2018collaborative, hong2019design, 10.1145/3290605.3300522}. 
Several studies in HCI, especially Computer-Supported Cooperative Work (CSCW) have built interactive systems and designs that apply in group work setting
~\cite{shahi2021amused, serrano2013cloud, hong2019design, amershi2008cosearch, bentley2017searchmessenger}. 
A line of work applies the spirit of ``the whole is greater than the sum of its parts'' in data annotation user interface design.
For instance, Chang et al.~\cite{10.1145/3025453.3026044} introduced a tool ``Revolt'' facilitating group decision-making for collaborative crowdsourced workers. 
They leveraged the disagreement between the annotators to identify ambiguous concepts and provide more options for decision-making based on the disagreement feedback, which has proven to be more efficient than the typical guideline-based approach. 
Upchurch et al. \cite{Upchurch_Sedra_Mullen_Hirsh_Bala_2016} present an online game allowing annotators to refine the majority vote labels to build consensus among them while labeling image data. 
Liu et al. \cite{10.1145/3544549.3573854} ran a case study investigating the utilization of multimodal data for assessing the interface in designing a collaborative reading system.

However, the underlying threat that makes group work \textit{less} than the sum of the individuals is highly associated with the knowledge gap. 
For instance, Kapania et al. \cite{10.1145/3544548.3580645} studied that when annotators lack access to essential information, clear guidance, and opportunities for collaboration, a knowledge gap can emerge among them. 
Expert annotators possess a deep understanding of the domain and context, enabling them to provide more accurate and consistent annotations whereas beginners may lack this critical expertise, leading to errors and misinterpretations in their annotations \cite{Robson_Searston_Edmond_McCarthy_Tangen_2020, wang2022ai, RUSSO2021117695}. 
%Annotation tasks are designed to establish a definitive ``ground truth'' label for training machine learning models, with the aim of minimizing the influence of annotators' individual subjectivities \cite{10.1145/3544548.3580645}. 
Crowdsourcing, a commonly employed method for labeling tasks involving crowd workers, such as Amazon's Mechanical Turk \cite{amazon}, predominantly relies on non-expert annotators \cite{10.1145/3290607.3313054, 10.5555/2491748.2491763, 10.1145/2047196.2047202}. 
Consequently, labeling carried out by individuals lacking expertise often proves challenging and tends to be error-prone. 
These discrepancies can hinder the development of robust machine learning models \cite{10.1145/1837885.1837906,10.1145/3290607.3313054}. 
Several studies also examined strategies for addressing ambiguity and disagreement during annotation, a crucial step in mitigating the knowledge gap. 
Kairam and Heer \cite{10.1145/2818048.2820016} applied an automated clustering-based method to identify divergent responses. 
Chen and Zhang \cite{chen2023judgment} introduce a new workflow, termed ``Judgment Sieve'', aiming at reducing uncertainty in tasks involving group judgment. 
They elicit different sources of uncertainty and apply targeted interventions, such as adding context or facilitating deliberation, to effectively reduce uncertainty. 
Chang et al. \cite{10.1145/3411764.3445165} suggest utilizing spatial layout to enhance the quality of labels in image annotation tasks performed by non-experts, which proved to be an efficient approach compared to non-spatial layout design. 

Human effort in data annotation in ML involves manually labeling or categorizing raw data, ensuring consistency and accuracy and often requires domain-specific expertise~\cite{abu2021domain}. 
%What are the aims of reducing human effort?
The nature of manual labeling and reliance on experts can make data annotation challenging to scale, standardize, and ensure consistent quality across large datasets.
%What are focused by past work 
Recognizing this challenge, past research has sought ways to alleviate the human burden in this domain. 
Researchers have proposed algorithmic enhancements like active learning to prioritize the most informative data points for annotation~\cite{chung2019efficient}, and semi-supervised learning to reduce the amount of labeled data needed~\cite{jain2021exploring, meudt2012atlas}. 
Chen et al. \cite{Chen_2021} introduce an elicitation algorithm for item rating that incorporates prior examples and leverages input from other annotators for pairwise comparisons. 
Their motivation for this active learning-based approach is to address the limitation that absolute scaling can exhibit inconsistency and unreliability.
Efforts in Alternative data sources where crowdsourcing distributes the annotation task among a larger group~\cite{song2019foureyes, song2018two}, synthetic data generation reduced the need for real-world labeled data~\cite{falcao2021piwims}.
Researchers have developed intuitive interfaces that simplify the task of labeling, incorporating features like drag-and-drop~\cite{shneiderman2000direct} or batch labeling~\cite{ashktorab2021ai}, highlighting~\cite{choi2019aila}, and leveraging language based models \cite{bai2022training}.
Desmond et al. \cite{10.1145/3397481.3450698} designed AI-assistive features using a semi-supervised technique to predict the labels. 
They used a non-AI assistive interface as a baseline and compared the performance with their proposed interface which shows AI-based system improved the speed and accuracy of the labels. 
Hierarchical approaches have also been adopted in designing annotation interfaces. 
Stureborg et al. \cite{Stureborg_2023} leveraged multiple schemes for crowdsourced multi-labeling tasks, i.e., grouping more similar contents together, filtering out negative examples, and different kinds of pass logic to coordinate between the crowdsourced annotators.
Gooding et al. \cite{gooding2023study} performed a comparative study on annotation interfaces for summarization tasks trained in-house annotators with backgrounds of different proficiency levels. 
From the annotator’s feedback the authors improvised the baseline interface applying the technique where tokens are highlighted on every instance upon user selection.

%BUT, only eprts why not novices? 
However, past research is focused on reducing human effort by minimizing the effort related to dealing with ground-truth~\cite{denton2021ground, hossain2017active, NEURIPS2020_b5d17ed2} with no attention to recruiting beginners who have less experience without complex training.
%In this work, aim at using gap to aid novices
In this work, we are interested in why beginners annotate inaccurately and understanding how this knowledge gap exists between beginners and experts could be used to arm beginners to perform like experts, especially in the disaster management context.
%
To the best of our knowledge, our work represents the first attempt to understand the knowledge gap between less experienced and experienced annotators regarding identifying crisis incidents and harness this knowledge to reduce human effort in data annotation while also improving the quality of annotations. 


%COMMENTED OUT
%\pq{I mentioned the types because collaboration usually has these types, and aim to show our work could be used in any case of collaboration. However, if this is useless. I will rewrite it by removing these categories.}
%This gap, which represents the difference in knowledge and expertise among group members, remains under-explored, especially in data annotation.
%In this user study, aim at using gap, mimic group work, improve
%The goal is to simulate the benefits of collaboration by allowing individuals to receive remote, asynchronous assistance but feel like in-person, synchronous assistance, thereby making their solo tasks more productive and effective.
%In that case, we propose integrating the knowledge gap between experts and novices into guidance, which could be referred unlimited by novices' solo use. 

% Group work is a collaborative effort where individuals come together to achieve a common goal~\cite{mattessich1992collaboration}.
% This kind of collaboration is omnipresent in our daily lives, from students working together to solve a problem~\cite{stahl2006computer}, to surgeons teaming for a complex procedure~\cite{torring2019communication}, to a group making decisions about future plans~\cite{fesenmaier2006destination, jameson2007recommendation, yue2014share}.
% Due to technological advancements, the boundaries of collaboration have expanded to allow for participation that is no longer bound by geographical proximity ~\cite{laaki2019prototyping, jin2023collaborative} or synchronous interactions~\cite{} \amandaIn{Need a citation that talks about synchronized collaboration, like shared document writing for example}. 
% \ray{Commented out two sentences below as they look irrelevant}
% \amanda{I think the two sentences by themselves were tangential, I worked a few of the ideas into the sentence above}
%Collaboration can occur in physical proximity, as demonstrated in endeavors like building construction~\cite{follini2020bim}, or it can reach beyond geographical boundaries, as evidenced by remote surgeries~\cite{laaki2019prototyping} and online classes~\cite{jin2023collaborative}. 
%Such collaborative efforts can take on various forms, whether they are synchronized, such as in live webinars~\cite{Zoom} and real-time competitions~\cite{blohm2011does}, or unsynchronized, as seen in shared document writing~\cite{}.


==> implementation.tex <==


\subsection{Implementation of interfaces}
\subsubsection{Highlight Interface}
In this interface, we highlight relevant and irrelevant tokens of the text to help the annotator pay more attention to the tokens that can potentially be indicative of the correct label. Moreover, we consider different intensities in highlighting the tokens to represent how much a token is relevant or irrelevant to the label. 
In our experiments, in the training phase, we use samples on which both expert and less-experience users agreed on the label in our previous study, and those samples on which both users disagreed are used for the testing phase. Therefore, to provide these tokens, we use samples from the agreement part to extract relevant and irrelevant tokens to each label, and calculate their relevancy measures, as follows:
\begin{enumerate}
    \item For each sample, we create a list of candidate tokens. These tokens include nouns, verbs, and named entities that exist in the sample. Here, we use Spacy to extract these tokens.
    \item To calculate the relevancy of each token to a class $C$, we exploit normalized Pointwise Mutual Information (nPMI) measure based on Eq. \ref{eq:1} and \ref{eq:2}. 
    \begin{equation} \label{eq:1} \tag{1}
        PMI(t,C) = \log \frac{p(t,C)}{p(t)p(C)} 
        
    \end{equation}
    \begin{equation} \label{eq:2} \tag{2}
        nPMI(t,C) = \frac{PMI(t,C)}{-\log_{2} p(t,C)} 
        
    \end{equation}
    where $p(t,C)$ is the probability of a sample containing token $t$ and is annotated as class $C$, $p(t)$ is the probability of a message containing token $t$, and $p(C$ is the probability of a message being annotated as class $C$. The normalized PMI measure which maps the PMI measure to the range of [-1,1] is used to measure the relevancy of the token $t$ to the class $C$, as:
    \begin{itemize}
        \item nPMI value of zero indicates no association between token $t$ and class $C$.
        \item A positive nPMI indicates that samples from class $C$ are more likely to use the token $t$.
        \item A negative nPMI indicates that samples from class $C$ are less likely to use the token $t$.
    \end{itemize}
    Furthermore, since we need to find both relevant and irrelevant tokens to the target class $C$, we divide the dataset into samples that have been annotated as \textit{relevant} to the target class $C$ and those with \textit{irrelevant} label. Therefore, we generate two lists of \textit{extracted relevant tokens} and \textit{extracted irrelevant tokens} to the class $C$ by calculating nPMI measure for each token in these two categories. In this way, higher $nPMI(t,C)$ on the relevant samples of class $C$ implies that the token $t$ is more relevant to class $C$, and higher $nPMI(t,C)$ on the irrelevant samples of class $C$ indicates that the token $x$ is less relevant to class $C$.
   
\end{enumerate}
In the testing phase, we highlight two tokens that are likely more relevant and two tokens that are likely less relevant to the class $C$. For selecting the top two relevant tokens, we use a list of \textit{expert-provided relevant tokens}  in addition to the list \textit{extracted relevant tokens} with the following procedure:
\begin{enumerate}
    \item If the candidate tokens in the test sample exist in the \textit{expert-provided relevant tokens}, they are selected and assigned a relevancy measure $nPMI=1.0$.
    \item We select top-k tokens from \textit{extracted relevant tokens} with the highest nPMI measures.
    \item We merge these two lists and select the top two tokens with the highest nPMI measures from the merged list.
\end{enumerate}
For selecting the top two less-relevant tokens, we use the list \textit{extracted relevant tokens} and select top-k tokens with the highest nMPI measures. Since it is possible that selected less-relevant tokens exist in the selected more-relevant tokens as well, we remove such tokens from the less-relevant list and select the top two tokens.

\subsubsection{Reasoning Interface}
In this interface, we provide reasoning about why or why not the current message can be relevant to a specific class. This helps the annotator to evaluate the sample from both perspectives and then select the class label for that sample. To generate the reasoning, we exploit the capabilities of Large Language Models (LLM) by prompting the model with the message and proper instructions. 
Since LLMs have been trained on a massive corpus they have good knowledge of subjects like \textit{Transportation Means}, but for the annotating task, we need to provide a definition of the subject that represents the annotation task's requirements, such as institutional insights. Moreover, LLMs usually generate long reasonings which can overwhelm the users with details that can confuse the users, so we need to provide short and informative reasoning. The procedure for generating reasoning by LLM is as follows:
\begin{enumerate}
    \item We prompt the LLM with the given tweet and expert-provided definition of class $C$, and ask the LLM to generate the reasoning about why the tweet is relevant or irrelevant to the class $C$.
    \item We extract all sentences from generated reasoning.
    \item Again, we prompt the LLM by providing these extracted sentences as the options and ask the LLM to select the reasoning from these options.
\end{enumerate}

\subsubsection{Context Interface}
In this interface, we propose two types of hints to address the knowledge gap and provide both in the interface. The first hint is specifying the tokens in the given sample that may cause ambiguity for the user to select the correct label. The second one is a reasoning based on the feedback from expert and less-experienced users, achieved from the previous study, that focuses on their disagreement. \\
To extract ambiguous tokens for a given label, we figure out the tokens from our dataset which are distributed almost equally in both relevant and irrelevant classes. However, these tokens need to occur at least \textit{min_freq} times in each class. For measuring the ambiguity of a token $t_k$ in a class $c_i \in \{\textit{relevant}, \textit{irrelevant}\}$, we calculate the ambiguity measure $AM(t_k, c_i)$ based on Eq.\ref{eq:3}:
\begin{equation} \label{eq:3} \tag{3}
        AM(t_k,c_i) = \frac{\mathit{tf} (t_k,c_i)}{\mathit{tf} (t_k)} 
        
\end{equation}
where $\mathit{tf}(t_k, c_i)$ is the frequency of token $t_k$ in class $c_i$, and  $\mathit{tf}(t_k)$ is the frequency of token $t_k$ in all classes. This measure represents the frequency of a token $t_k$ in each class, so to measure the ambiguity of token $t_k$ in the given label, we calculate the  ambiguity measure $AM(t_k)$ based on Eq.\ref{eq:4}
\begin{equation} \label{eq:4} \tag{4}
        AM(t_k) = \underset{c_i}{\mathrm{argmax}} (AM(t_k, c_i))
        
\end{equation}
If a token $t_k$ equally occurs in both relevant and irrelevant classes, the ambiguity measure $AM(t_k)=0.5$, which means the token has the highest ambiguity. If the token occurs only in one class, the ambiguity measure is equal to 1.0 which implies that the token is indicative of a particular class, so it is not ambiguous at all. Therefore, the range of ambiguity measure is [0.5, 1.0]. We set a threshold \textit{max_amb} (0.7 in our experiments), and tokens with $AM(t_k) \leq max\_amb$ are considered as ambiguous tokens. \\
In our experiment, we use the samples from the disagreement part of the dataset, as the training set, to figure out ambiguous tokens for each label (Transportation means or Damaged infrastructure), since these samples can represent the knowledge gap between expert and less-experienced users. First, we calculate the ambiguity measure for all tokens in the training set and then select the top-k (k=3 in our experiment) token with the lowest $AM$ measure (higher ambiguity).
To provide reasoning about the knowledge gap between users based on their feedback, we prompt an LLM with the test sample, selected labels by the users for that sample, and their feedback regarding their choice and ask the model to generate reasoning. We generate the reasoning for a given sample through the following steps:
\begin{enumerate}
    \item For each annotator, we prompt the LLM with the text, the definition of the label, and the annotator's feedback and ask the LLM to generate reasoning behind the annotator's prediction. We use the prompt in Figure \ref{fig:prompt-reasoning-generator} for this purpose. Providing the definition of the label helps the LLM to consider institutional insights in generating the reasoning.
    \item  We prompt the LLM with the text, the definition of the label, and two reasoning generated in step (1) and ask the model to generate the reason behind the users' disagreement. We change the order of providing annotators' reasoning to eliminate any bias that may caused by the order. We use the prompt in Figure \ref{fig:prompt-context-generator} in this step.

\end{enumerate}

\begin{figure}[!htb]
  \centering
\fbox{\begin{minipage}{15em}

\textbf{Instruction:} Read the definition and the annotator's reasoning about the following tweet and complete the answer. 

\textbf{Definition:} <given-definition>

\textbf{Tweet:} <given-tweet>

\textbf{Annotator:} <annotator-feedback>

\textbf{Answer:} Annotator believes that the tweet is <annotator-prediction> to <disagreement-label> because

\end{minipage}}
\caption{Prompt for generating reasoning based on the user's feedback}
\label{fig:prompt-reasoning-generator}
\end{figure}

\begin{figure}[!htb]
  \centering
\fbox{\begin{minipage}{15em}


\textbf{Instruction:} Two annotators generated the following reasonings for the following task and tweet. What is the reason for their
disagreement? 

\textbf{Task:} Based on the following definition, is the following tweet relevant to <disagreement-label>?

\textbf{Definition:} <given-definition>

\textbf{Tweet}: <given-tweet>

\textbf{Annotator 1:} <annotator1-reasoning>

\textbf{Annotator 2:} <annotator2-reasoning>

\textbf{Answer:} The reason for their disagreement is that


\end{minipage}}
\caption{Prompts for generating reasoning behind the users' disagreement}
\label{fig:prompt-context-generator}
\end{figure}
